Understanding the Information Propagation Effects of Communication Topologies in LLM-based Multi-Agent Systems

The communication topology in large language model-based multi-agent systems fundamentally governs inter-agent collaboration patterns, critically shaping both the efficiency and effectiveness of collective decision-making. While recent studies for communication topology automated design tend to construct sparse structures for efficiency, they often overlook why and when sparse and dense topologies help or hinder collaboration. In this paper, we present a causal framework to analyze how agent outputs, whether correct or erroneous, propagate under topologies with varying sparsity. Our empirical studies reveal that moderately sparse topologies, which effectively suppress error propagation while preserving beneficial information diffusion, typically achieve optimal task performance. Guided by this insight, we propose a novel topology design approach, EIB-leanrner, that balances error suppression and beneficial information propagation by fusing connectivity patterns from both dense and sparse graphs. Extensive experiments show the superior effectiveness, communication cost, and robustness of EIB-leanrner.

==> sec1_v1_backup.tex <==
Agents powered by large language models (LLMs) ~\cite{li2023camel,wang2024survey,xi2025rise} have demonstrated strong performance across tasks like reasoning~\cite{yao2023react}, code generation~\cite{zhang2024codeagent}, and complex decision-making~\cite{guo2024embodied}. A key advancement in this area is the development of collaborative \textbf{multi-agent systems (MAS)}, where multiple LLM agents interact to outperform single-agent when tackling complex tasks~\cite{talebirad2023multi,liang2024encouraging,guo2024large,li2023theory}. While role specialization contributes to this improvement~\cite{bo2024reflective}, the communication topology, which defines how agents exchange information, plays a more fundamental role in enabling effective collaboration~\cite{qian2024scaling,zhang2024exploring}. From simple chain~\cite{zhang2024chain} and tree~\cite{zhou2024language}, to fully connected graphs~\cite{hu2024learning} and LLM-generated designs~\cite{zhuge2024gptswarm}, prior works have proposed various topologies to guide this interaction. These studies converge on a central insight: \textbf{\textit{the topology of communication is critical to the accuracy, efficiency, and final performance of multi-agent systems}}.
\begin{figure}[t!]   

\centering    
% 前面说过，图片放置在中间
	\includegraphics[scale=0.3]{fig/intro.pdf}
			
					\caption{Illustration of insight suppression caused by chain (top) and error propagation induced by fully connected topologies (bottom).}
      % 整个图片的说明，注释写在{}内
					\label{fig:intro}  
\vskip -1 em
\end{figure}

Building on this, recent works have shifted from manually designed topologies to learning-based approaches that aim to induce sparse communication structures, motivated by the belief that fewer but more informative interactions can improve efficiency~\cite{li2024improving,liu2025advances,zhou2025multi}. For example,~\cite{zhang2024cut} learns a task-specific sparse mask to eliminate suboptimal connections, while~\cite{wang2025agentdropout} introduces stochastic  pruning on both nodes and edges to encourage sparsity robustness. ~\cite{zhang2024g} goes further by generating a query-dependent sparse graph to improve adaptability. While these methods do lead to performance gains and reduced token costs, they often treat sparsity as an end goal, without addressing a deeper question: \textbf{why} and \textbf{when} does sparsity help or hurt collaboration? This lack of explanation motivates a more fundamental investigation: Instead of simply learning sparser topologies,  \textbf{\textit{how different communication structures, whether sparse or dense, causally affect the reasoning and decision-making capacity of multi-agent systems}}.

%Compared to manually crafted communication topology, recent state-of-the-art methods have begun to explore learning-based approaches that automatically derive task-specific topologies. These methods primarily aim to improve communication efficiency by removing redundancy, often under the assumption that \textbf{fewer interactions can yield similar or even better performance.} For instance, Cut the Crap proposes learning a sparse but fixed mask tailored to each task, which selectively disables certain inter-agent connections during inference to avoid reliance on suboptimal communication. AgentDropout extends this idea by introducing stochastic dropout on both nodes and edges, further encouraging sparse and robust interaction patterns. In contrast to learn a single fixed structure per task, G-Designer employs a graph generator to produce a unique sparse topology for each individual query, thereby enhancing adaptability across varying input scenarios. While these approaches offer practical benefits in terms of computational and economic cost, they share a common focus: they treat sparsity as an end goal, \textbf{without explaining why or when sparse structures actually help or hurt multi-agent collaboration.}
%This lack of explanation motivates a deeper investigation: instead of simply learning sparser topologies, \textbf{\textit{how to understand the causal relationship between a communication structure, whether sparse or dense, and the collective decision-making performance of the multi-agent system.}}

% In this paper, we propose a causal analysis framework that investigates how the correctness of an individual agent's output—whether accurate or erroneous—propagates through different communication topologies and ultimately influences the collective decision of the multi-agent system. Specifically, we design two counterfactual intervention strategies: error injection and answer injection. These interventions enable us to quantitatively evaluate the impact of both correct and incorrect agent-level outputs under varying topological structures. By systematically comparing sparse and dense communication structures, we reveal that sparser topologies are more effective at suppressing the influence of erroneous information, thereby enhancing robustness, while denser topologies facilitate the rapid dissemination of correct answers, promoting consensus and accuracy. These observations lead to a central insight: \textbf{\textit{the optimal communication structure is not the sparsest or the densest, but one that suppressing error propagation while preserving efficient information sharing.}}
In this paper, We propose a causal analysis framework to examine how individual agent outputs, whether accurate or erroneous, propagate under different communication structures. We design two counterfactual interventions, error injection and answer injection, to analyze how the topology affects the propagation of misinformation and the retention of insightful content. These two processes are illustrated in Figure~\ref{fig:intro}. We further introduce a metric, Total Counterfactual Topology Effect (TCTE), specifically designed to measure how different communication topologies respond to the two counterfactual interventions. Our experiments reveal that moderately sparse topologies better suppress error propagation, while moderately dense ones more effectively retain and transmit insightful information.
This leads to a novel insight: \textbf{\textit{the optimal communication topology is not the sparsest or the densest, but one that suppressing error propagation while preserving efficient insight sharing.}}

% Building upon this insight, we propose a graph neural network (GNN)-based architecture to emulate the message-passing process among agents. We begin with a fully connected graph as a message-passing template and identify a subgraph composed of nodes and links that are critical for the rapid dissemination of correct information. In parallel, we use a chain graph as another structural template to extract the subgraph most effective at suppressing the propagation of erroneous information. By fusing these two subgraphs, we obtain a task-specific communication topology that enables rapid convergence to a correct consensus and robustness to erroneous occurs, enabling reliable and efficient collective decision making. To sum up,the main contributions of this paper are as follows:
% Building on this insight, we propose a novel topology learning framework that explicitly incorporates the dual structural objectives revealed by our causal analysis: suppressing error propagation and preserving informative signals. We model multi-agent communication as a message-passing process over a graph and use a Graph Neural Network (GNN) as a simulator to learn how information flows under different topologies. To capture different propagation dynamics, we construct two soft connectivity masks: one from a fully connected graph to support efficient information diffusion, and one from a chain structure to enforce cautious propagation. A query-aware fusion module then adaptively combines these two views based on task semantics, yielding a task-specific communication topology. 
Based on our causal findings, we introduce \textbf{D}ual-view \textbf{C}ommunication \textbf{T}opology \textbf{L}earning (\ourmethod for short), a topology generation framework tailored for multi-agent systems powered by LLMs. \ourmethod models agent communication as a message-passing process over a graph, using a Graph Neural Network (GNN) to simulate information flow. To explicitly capture the dual objectives revealed by our causal analysis, \ourmethod learn two soft connectivity masks: one from a dense view to promote the spread of correct information, and another from a sparse view to limit error propagation. A query-aware fusion module then adaptively integrates the two views to generate a task-specific topology. This enables the MAS to remain robust in the presence of error while effectively leveraging informative insight, supporting more accurate and stable group decision-making.
% Building on this insight, we propose a topology learning framework that explicitly reflects the dual objectives identified by our causal analysis. We model multi-agent communication as a message-passing process over a graph, using a Graph Neural Network (GNN) to simulate information flow under different topologies. To capture distinct propagation dynamics, we construct two soft connectivity masks: one from a fully connected graph to facilitate insightful information propagation, and another from a chain structure to restrict the spread of errors. A query-aware fusion module then adaptively combines these views based on task semantics, generating a task-specific topology that balances efficiency and robustness. This design enables the MAS to converge quickly when agent inputs are reliable while remaining resilient to misleading information, ultimately supporting more accurate and stable collective decision making.

 To sum up,the main contributions of this paper are as follows:
 \begin{itemize}
    \item \textbf{Causal Analysis of Communication topologies:} We propose a causal counterfactual analysis framework to assess the impact of an agent on collective decision making across various communication topologies, revealing how communication sparsity and density influence the collaboration between agents.
    % \item \textbf{Topology Learning Guided by Causal Insights:} We develop a GNN-based framework that learns task-specific communication topologies by integrating two soft connectivity masks designed to suppress errors and preserve insightful signals, guided by causal analysis.
    \item \textbf{Topology Learning Guided by Causal Insights:} We propose \ourmethod, a GNN-based framework that simulates multi-agent communication and learns dual-view soft connectivity masks guided by our causal analysis, and adaptively fuses them into task-specific topologies.
    \item \textbf{Comprehensive Empirical Validation:} Extensive experiments on six multi-agent decision-making benchmarks demonstrate that our method achieves superior accuracy with reduced communication cost compared to existing baselines.
\end{itemize}

==> sec3_v1_backup.tex <==
While prior graph-based multi-agent system (MAS) designing approaches primarily focus on producing sparse communication topologies to reduce redundancy, it is not clear how these topologies shape the actual information flows between agents and influence the results of collective decisions. This motivates us to delve into the topology factors that govern communication effectiveness. To this end, we try to answer two interrelated sub-questions (SQs) that together capture the dual role of topologies in modulating information flows in MAS. \textbf{\textit{SQ1}: How does the communication topology mediate the spread of errors?} Concretely, when an individual agent accidentally produces incorrect information, does the topology amplify this error and lead the group to a wrong decision? \textbf{\textit{SQ2}: How does the communication topology shape the propagation of accurate information?} Conversely, when an agent generates accurate and helpful insight, does the topology enable its influence to be retained and integrated into the final output, or is it suppressed along the way? These considerations lead us to our central research focus: \textbf{\textit{In a MAS, how different topologies affect its vulnerability to error propagation and its ability to preserve beneficial information.}}

\subsection{Causal Metric}

In order to answer the above questions, it is crucial to quantify the impact of each agent on the whole MAS, which allows us to systematically analyze how agent-level errors or accurate information propagate through the network and ultimately affect collective outcomes. 
To this end, we first introduce a new metric from the causal perspective, denoted as Counterfactual Agent Propagation Effect (\textbf{CAPE} for short), which quantifies the causal influence of a single agent’s output on the system’s final answer under a given communication graph. Specifically, we perform a counterfactual intervention by forcing agent $v_{i}$ to produce a deliberately manipulated output, and then measure whether this change alters the final prediction made by the MAS under a fixed topology $\mathcal{G}$. The formal definition is as follows:
\begin{definition}
   Given a MAS under communication graph $\mathcal{G}$, for a query $\mathcal{Q}$, let $y_{Q}^\text{orig} \in \{0,1\}$ denote whether the final system answer is correct under the original communication process. The Counterfactual Agent Propagation Effect {\text{(CAPE)}} of agent $v_i$ under $\mathcal{G}$ and query $\mathcal{Q}$ as:
   \begin{align}
       \resizebox{.8\hsize}{!}{$\textbf{CAPE}_{i}(\mathcal{G},\mathcal{Q}) = \mathbb{I}[y_q^{\text{cf}}(\mathcal{G}, \text{do}(\mathcal{O}_i := \hat{\mathcal{{O}}}_i)) \ne y_q^{\text{orig}}(G)]$},
   \end{align}
   where $ \operatorname{do}(\mathcal{O}_i := \hat{\mathcal{{O}}}_i))$ denotes a targeted intervention that forces only agent $v_{i}$ output to a counterfactual value $\hat{\mathcal{{O}}}_i$, $y_{\mathcal{Q}}^{\text{cf}} \in \{0,1\}$ is the correctness of the final system prediction after the intervention, and $\mathbb{I} \left[ \cdot
\right]$ is the indicator function for whether the final answer of MAS is flipped.
\end{definition}
% CAPE captures how the communication structure mediates the spread of local agent interventions to global system behavior, allowing us to diagnose whether a topology amplifies or dampens the effects of agent-level errors or insights. 
A higher {CAPE} value suggests that changes in an individual agent’s output, once propagated through the communication structure, have a stronger influence on the final decision of MAS. Building on the ability of CAPE to quantify agent-level influence, we further define the Total Counterfactual Topology Effect (TCTE) to aggregate these effects at the topology level, providing a comprehensive measure of the general sensitivity of the topology to localized interventions.
\begin{definition}
Given a communication topology $\mathcal{G}$, the Total Counterfactual Topology Effect (\textbf{TCTE}) for query $\mathcal{Q}$ is defined as:
\begin{align}
\text{TCTE}(\mathcal{G},\mathcal{Q}) = \frac{1}{N}\sum_{v_i\in V} \frac{1}{\sqrt{d_i}} \cdot \text{CAPE}_{i}(\mathcal{G},\mathcal{Q}),
\end{align}
where $d_i$ is the degree of agent $v_i$ in graph $\mathcal{G}$. 
\end{definition}

In TCTE, the $1/\sqrt{d_i}$ factor downweights the agents with high degree, reflecting the intuition that highly connected agents are more likely to spread influence, and we wish to normalize their impact accordingly. A higher TCTE indicates that the topology is more responsive to specific changes in agent-level output, implying a greater potential to either propagate erroneous information or effectively transmit correct insights.
% Intuitively, a higher \textbf{TCTE} indicates that the system is more sensitive to localized changes—errors or corrections—suggesting a topology that more strongly amplifies agent-level perturbations. Conversely, a lower TCTE suggests that the structure acts as a dampening medium, making the system more robust to individual deviations. By comparing TCTE values across topologies, we can quantitatively analyze how structural properties—such as sparsity or connectivity—affect the collective decision-making dynamics of the system.
% This helps us analyze how different topologies modulate the influence of both beneficial and harmful agent-level information on the final system output.
\subsection{Validation Experiments and Analysis}
In this subsection, we aim to empirically assess how different communication topologies affect the sensitivity of MAS to agent-level perturbations. We quantify the sensitivity by computing TCTE across a range of graph structures, thereby answering our sub-questions, i.e. \textbf{\textit{SQ1}} and \textbf{\textit{SQ2}}.

\begin{figure}[t]
  \centering
  % 第一行：两张并排
  \subfloat[Error propagation]{%
    \label{subfig:error}%
    \includegraphics[
      width=0.5\columnwidth,
    ]{fig/CAPE_error.pdf}%
  }\hfill
  \subfloat[Insight suppression]{%
    \label{subfig:insight}%
    \includegraphics[
      width=0.5\columnwidth,
    ]{fig/CAPE_answer.pdf}%
  }

  \vspace{-1em} % 两行之间垂直间距

  % 第二行：一张拉伸到底栏宽
  \subfloat[Impact of all baseline topology]{%
    \label{subfig:baselinetp}%
    \includegraphics[
      width=\columnwidth
    ]{fig/CAPE_baseline.pdf}%
  }

  \caption{Experimental validation of how different communication topologies affect error propagation and the transmission of useful insight, as quantified by TCTE under two types of counterfactual interventions.}
  \label{fig:three_plots}
  \vskip -1 em
\end{figure}

\subsubsection{Experimental Settings}
% \noindent \textbf{Experimental Settings} \ \ \ 
% We conduct experiments on the MMLU dataset. For each topology, we select 500 questions that are originally answered correctly and 500 that are answered incorrectly by the multi-agent system. To create structures with varying sparsity, we start from a fully connected graph with six agents and randomly remove edges to construct topologies with different levels of sparsity. To evaluate error propagation, we perform a counterfactual intervention by forcibly modifying an agent’s prompt to produce an incorrect and misleading output, i.e., $\hat{o}_{i} = \text{error}$. This intervention is applied to the 500 originally correct questions, and $\text{CAPE}^{\text{error}}$ is computed to measure how often these injected errors flip the final system prediction.
% We conduct experiments on the MMLU dataset to evaluate how different communication topologies affect the system’s response to both harmful and beneficial agent-level perturbations. For each topology, we select 500 questions that are originally answered correctly and 500 that are answered incorrectly by the multi-agent system. To construct structures with varying connectivity, we manipulate the topology in two ways: starting from a fully connected graph with six agents, we progressively remove edges to simulate increasing sparsity; conversely, starting from a sparse chain graph, we gradually add edges to enhance connectivity. To evaluate error propagation, we apply a counterfactual intervention by modifying an agent’s prompt to produce incorrect output, i.e., $\hat{o}{i} = \text{error}$, and compute $\text{CAPE}^{\text{error}}$ on the 500 originally correct questions to measure how often the system’s prediction flips to incorrect. To assess the amplification of correct information, we inject the correct answer into the prompt of a selected agent, i.e., $\hat{o}{i} = \text{answer}$, on the 500 originally incorrect questions and compute $\text{CAPE}^{\text{answer}}$ to evaluate how often the system recovers the correct prediction.
We conduct our experiments on the MMLU dataset, a benchmark for evaluating knowledge and reasoning across diverse domains. In our multi-agent setup, each of the six agents is an independent instance of GPT-3.5 with a distinct role and prompt template, and all communicate according to a pre-specified topology graph. For each topology, we construct two evaluation sets: one containing 500 questions that the multi-agent system originally answers correctly, and another with 500 questions that the system answers incorrectly. These sets serve as the basis for simulating both detrimental and beneficial agent-level interventions under varying graph structures.

% \noindent \textbf{} \ \ \  
\subsubsection{Analysis of Error Propagation}

\noindent \textbf{Setup.} \ \ \
To address \textbf{\textit{SQ1}}, we focus on the 500 originally correct questions and assess the vulnerability of MAS to local errors under varying topologies. We start from a fully connected communication graph and progressively remove edges randomly to generate topologies with different sparsity levels. We then apply a counterfactual intervention by modifying the system prompt of the agent to produce an incorrect output, i.e., $\hat{\mathcal{{O}}}_i = \text{error}$, and compute the corresponding $\text{TCTE}$ to quantify how often the final prediction flips from correct to incorrect under each topology. 

\noindent \textbf{Discussion of Results.} \ \ \
As shown in Figure \ref{subfig:error}, dense topologies are significantly more vulnerable to what we refer to as error propagation, where an incorrect output from a single agent is more likely to influence the system's overall decision. When the sparsity is zero (i.e., a fully connected graph), $\text{TCTE}$ reaches its peak. In contrast, sparser structures can effectively mitigate this issue. For example, in the extreme case of a chain topology, $\text{TCTE}$ is reduced by up to $19\%$, indicating improved robustness to localized errors. Moreover, moderate sparsity also contributes to better task performance: as sparsity increases from 0 to 0.4, the system’s accuracy improves by up to $3.2\%$. Based on the above experimental results, we arrive at the following conclusion.
\begin{tcolorbox}[
    enhanced, % 启用增强样式
    colback=white, % 背景色（白色）
    colframe=black, % 边框颜色（黑色）
    boxrule=1pt, % 边框线宽
    arc=5pt, % 直角边框（无圆角）
    left=5pt, right=5pt, % 左右内边距
    top=5pt, bottom=5pt, % 上下内边距
    width=\linewidth % 宽度与文本等宽
]
\textbf{Conclusion 1:} Moderately sparse topologies mitigate the risk of error propagation within the system.
\end{tcolorbox}
%To address subquestion 1, we simulate the injection of erroneous information by performing a counterfactual intervention: we forcibly modify an agent’s prompt to produce an incorrect and misleading output. This intervention is applied to the 500 questions originally answered correctly. CAPE is then computed to quantify how often such injected errors change the system’s final decision from correct to incorrect. As shown in Figure 3, denser communication structures are more susceptible to what we term error propagation, where incorrect outputs from individual agents are more likely to influence the overall decision. %而稀疏的结构能避免

% To address subquestion 2, we again use prompt-based counterfactual intervention—this time injecting the correct answer into a selected agent. This intervention is applied to the 500 questions that were originally answered incorrectly. CAPE is computed to capture how often this injected correct information flips the system’s decision from incorrect to correct. As illustrated in Figure 3, we observe that sparser structures are more prone to what we call answer suppression, where structural constraints limit the dissemination of correct information, preventing it from improving the system’s output. %而稠密的系统可以快速传播答案
% \subsection{Analysis of insight suppression}
% \noindent \textbf{Experimental Settings} \ \ \ We conduct experiments on the MMLU dataset. For each topology, we select 500 questions that are originally answered correctly and 500 that are answered incorrectly by the multi-agent system. To evaluate the effect of information amplification, we start from a sparse chain graph and progressively increase connectivity by randomly adding edges, thus creating topologies with different levels of connectedness. For the 500 originally incorrect questions, we perform a counterfactual intervention by injecting the correct answer into the prompt of a selected agent, i.e., $\hat{o}_{i} = \text{answer}$. We then compute $\text{CAPE}^{\text{answer}}$ to measure how often this injected correct information changes the system’s final prediction from incorrect to correct.
\subsubsection{Analysis of Insight Suppression}

\noindent \textbf{Setup.} \ \ \ To address \textbf{\textit{SQ2}}, we examine how different topologies support the propagation of beneficial insight. We focus on the 500 originally incorrect questions and start from a sparse chain topology, gradually adding edges to increase connectivity. In each case, we perform a counterfactual intervention by injecting the correct answer into a selected agent’s prompt, i.e., $\hat{\mathcal{{O}}}_i = \text{answer}$, and compute the corresponding $\text{TCTE}$ to measure how often the system’s prediction flips from incorrect to correct.

\noindent \textbf{Discussion of Results.} \ \ \
As shown in Figure \ref{subfig:insight}, sparse topologies are more susceptible to what we term insight suppression, where too sparse topologies impede the propagation of accurate and informative signals, preventing them from influencing the final output. When connectivity is minimal (i.e., a chain), $\text{TCTE}$ reaches its lowest value, indicating poor transmission of correct insights. In contrast, this limitation is alleviated as the network becomes more connected. For example, in the extreme case of a fully connected topology, $\text{TCTE}$ increases by $10.5\%$, suggesting that the system becomes more capable of integrating accurate agent-level inputs into the final decision. Moreover, we observe that moderate density also contributes to improved task performance: as connectivity increases from 0 to 0.4, the system’s accuracy improves by up to $1.01\%$.  Based on the above experimental results, we arrive at the following conclusion.
\begin{tcolorbox}[
    enhanced, % 启用增强样式
    colback=white, % 背景色（白色）
    colframe=black, % 边框颜色（黑色）
    boxrule=1pt, % 边框线宽
    arc=5pt, % 直角边框（无圆角）
    left=5pt, right=5pt, % 左右内边距
    top=5pt, bottom=5pt, % 上下内边距
    width=\linewidth % 宽度与文本等宽
]
\textbf{Conclusion 2:} Moderately dense topologies enhance the system’s ability to rapidly propagate correct insights.
\end{tcolorbox}
%通过对现有的预定义结构的分析以及可学习的两个方法的分析，我们发现他们都无法在答案传播和错误阻碍这两部分取得平衡。多智能体的协作的核心在于求同存异，即当大多数agent趋向于正确答案时能够快速得到统一答案，当少数agent出现错误时能被抑制。需要一个恰好平衡的结构，为产生正确答案的智能体构建稠密的链接从而将正确答案快速传播，为产生错误答案的智能体构建瓶颈，从而抑制他的传播。
\subsubsection{Analysis of Existing topologies}
We evaluate a range of representative communication topologies, including pre-defined topologies such as \texttt{Full}, \texttt{Layered}, \texttt{Random}, \texttt{Star}, and \texttt{Chain}, as well as topologies learned through recent methods such as \texttt{AgentDrop} and \texttt{AgentPrune}. Following the experimental setup described above, we perform agent-level interventions based on both erroneous and correct outputs for each topology and compute the corresponding \text{TCTE}. As shown in Figure \ref{subfig:baselinetp}, the results reveal a consistent trend: sparse topologies are more robust to error propagation, while denser structures better support the amplification of helpful insight, which echoes our earlier analysis. However, no single topology achieves strong performance on both objectives simultaneously. Notably, the best-performing structures in terms of overall task accuracy are neither the sparsest nor the densest, suggesting that effective multi-agent communication requires a balanced topology that can simultaneously suppress error propagation and preserve the transmission of informative insight. These observations lead us to the following insights:
\begin{tcolorbox}[
    enhanced, % 启用增强样式
    colback=white, % 背景色（白色）
    colframe=black, % 边框颜色（黑色）
    boxrule=1pt, % 边框线宽
    arc=5pt, % 直角边框（无圆角）
    left=5pt, right=5pt, % 左右内边距
    top=5pt, bottom=5pt, % 上下内边距
    width=\linewidth % 宽度与文本等宽
]
\textbf{Final Conclusion:} An effective topology should build dense connections around agents likely to produce correct answers to amplify their influence, while creating structural bottlenecks around potentially erroneous agents to limit the spread of misinformation.
\end{tcolorbox}

==> sec4_v1_backup.tex <==
In this section, we present our proposed method, \textbf{D}ual-view \textbf{C}ommunication \textbf{T}opology \textbf{L}earning (\ourmethod). This approach is motivated by the insight that effective communication topologies in multi-agent systems should both amplify beneficial insight and suppress the spread of errors. While our evaluation metric TCTE captures this trade-off, it is a post-hoc diagnostic tool that requires ground-truth answers and is therefore impractical during system deployment. To overcome this limitation, \ourmethod introduces a topology generation framework that employs Graph Neural Networks (GNNs) to simulate multi-agent communication (Section \ref{GNN}), generate two topology masks from dense and sparse views to suppress errors and enhance correct insights respectively, and adaptively fuse them via a query-aware mechanism (Section\ref{dual_graph}).

\subsection{GNN as Simulator}\label{GNN}

To model how information propagates within a multi-agent system under a given communication topology, we use a Graph Neural Network (GNN) to simulate the message passing process. The Execution paradigm of GNNs inherently corresponds to multi-agent communication, with agents represented as nodes and edges denoting communication links.

Formally, at each GNN layer $L$, the message representation for node $v$ is updated by aggregating features from its neighbors:
\begin{equation}\label{message-passing}
\resizebox{.85\hsize}{!}{$\mathbf{m}_{v}^{(L)} = \operatorname{MP}\left (\mathbf{m}_{v}^{(L-1)},\{ \mathbf{m}_{u}^{(L-1)} \mid u \in \mathcal{N}(v) \} \right),$}
\end{equation}
where $\mathbf{m}^{(0)}_v = \mathbf{X}_v$ is the raw input feature of node $v$, $\mathcal{N}(v)$ denotes the set of neighbors, and $\operatorname{MP}$ is the message passing function that aggregates and integrates neighborhood information.

To initialize node features, we first encode each agent’s input representation by combining the textual description of its assigned role with the current task query:
\begin{align}
	\mathbf{x}_i \leftarrow \text{NodeEncoder}(\mathcal{T}(\text{Role}_i), \text{Query}),
\end{align}
where $\mathcal{T}(\cdot)$ extracts the textual description of the current agent’s role and its corresponding prompt. The \texttt{NodeEncoder} can be implemented using lightweight text embedding models. This design aligns with the input format used in the multi-agent system as shown in Eq. \ref{mp_in_multi-agent}, where each agent receives a prompt composed of both its designated role and the current query.

% Through this simulation process, the GNN learns which connections and node features contribute most to accurate final predictions, enabling us to infer structural patterns that facilitate effective information propagation.

\subsection{Topology Generator via Dual-Graph Encoding}\label{dual_graph}
% To be completed
% \subsection{Topology Generator via Dual-Graph Encoding}
% To construct a topology that effectively balances error suppression and answer propagation, we propose a structure generator based on dual-graph encoding. Motivated by our previous analysis as shown in \textbf{Conclusion 1} and \textbf{2}, we leverage these complementary characteristics to guide the learning of favorable nodes and links that support correct information flow and suppress harmful signals.
To identify an effective communication topology that balances suppression of error (\textbf{Conclusion 1}) and insight propagation (\textbf{Conclusion 2}), we adopt a GNN-based autoencoder framework to generate a soft adjacency mask $\mathbf{M}$ over the agent interaction graph. Given an input adjacency matrix $\mathbf{A}$ and corresponding agent features $\mathbf{X}$, the generator applies a message-passing encoder to produce latent node representations, followed by an inner-product decoder to estimate pairwise connectivity:
\begin{equation}
    \mathbf{Z} = \operatorname{GNN}(\mathbf{A},\mathbf{X}), \mathbf{M} =  \sigma(\mathbf{Z}^{T}\mathbf{Z}),
\end{equation}
where $\sigma(\cdot)$ denotes the sigmoid function to ensure outputs are in $[0, 1]$.
To capture different topological biases, we instantiate this module twice using two predefined templates: a fully-connected graph $\mathbf{A}_{\text{dense}}$ that encourages answer diffusion, and a chain-structured graph $\mathbf{A}_{\text{sparse}}$ that emphasizes cautious, localized propagation. These yield two connectivity masks, $\mathbf{M}_{\text{dense}}$ and $\mathbf{M}_{\text{sparse}}$, which serve as the basis for fusion and final graph construction.

To generate a final adaptive topology that integrates the strengths of both dense and sparse perspectives, we introduce a simple yet effective fusion function:
\begin{equation}
\mathbf{M}_{\text{final}} = \operatorname{Fuse}(\mathbf{M}_{\text{dense}}, \mathbf{M}_{\text{sparse}}).
\end{equation}
The fusion function is designed to softly weight the two structural masks in a query-aware manner. Specifically, we employ a gating-based mechanism that takes the task query embedding $\mathcal{Q}$ as input and dynamically computes the combination of the two views. This mechanism captures high-level semantic dependencies between the query and structural preferences, allowing the system to favor either rapid propagation (dense) or cautious suppression (sparse) depending on task context.

Formally, we instantiate the fusion weights $\mathbf{\alpha} = [\alpha_{\text{dense}}, \alpha_{\text{sparse}}]$ using a lightweight feedforward gating network:
\begin{equation}
\alpha = \text{softmax}(\mathbf{W}_2 \cdot \text{ReLU}(\mathbf{W}_2 \mathcal{Q}+ \mathbf{b}_1) + \mathbf{b}_2),
\end{equation}
where $\mathbf{W}_1$, $\mathbf{W}_2$, $\mathbf{b}_1$, and $\mathbf{b}_2$ are learnable parameters. The final mask is then computed as:
\begin{equation}
\mathbf{M}_{\text{final}} = \alpha_{\text{dense}} \cdot \mathbf{M}_{\text{dense}} + \alpha_{\text{sparse}} \cdot \mathbf{M}_{\text{sparse}}.
\end{equation}
% The resulting $M_{\text{final}}$ is then directly adopted as the multi-agent communication topology, guiding the message-passing structure among agents during downstream reasoning. 
%Intuitively, it balances the advantages of dense propagation for answer transmission and sparse masking for error suppression, forming an adaptive and task-aware communication graph $\mathcal{G}_{\text{com}}$.
The final mask $\mathbf{M}_{\text{final}}$ is used to sample a discrete communication topology $\mathcal{G}$ that determines how messages flow between agents during inference, following the  edge sampling strategy proposed in~\citet{zhang2024cut}.

To optimize this structure generation process, we aim to maximize the utility of the resulting communication topology, which measures the correctness  the final output $\mathcal{O} = \mathcal{G}(\mathcal{Q}) $ under the learned communication topology. However, the utility function $\phi(\cdot)$ is typically non-differentiable under our task setting sicnce depends on downstream black-box reasoning (e.g., querying LLMs), we adopt the standard policy gradient method to estimate gradients and update model parameters:
% \begin{align}
% \nabla_{\Theta}\mathbf{E}_{\Theta\sim\Omega}\Big[\phi\big(\mathcal{G}(\mathcal{Q})\big)\Big]\approx \frac{1}{M}\sum_{m=1}^{M}\phi(\mathcal{O}_{m})\nabla_{\Theta}\log(P(\mathcal{G}_{m})),
% \end{align}
\begin{equation}
       \resizebox{.85\hsize}{!}{$\nabla_{\Theta}\mathbf{E}_{\Theta\sim\Omega}\Big[\phi\big(\mathcal{G}(\mathcal{Q})\big)\Big]\approx \frac{1}{M}\sum_{m=1}^{M}\phi(\mathcal{O}_{m})\nabla_{\Theta}\log(P(\mathcal{G}_{m}))$},
   \end{equation}
where the $\Theta\sim\Omega$ are learnable parameters in \ourmethod, $P(\mathcal{G}_{m})$ calculates the probability of $\mathcal{G}_{m}$ being sampled. $\phi(\mathcal{O}_{m})$ can be treated as the task-specific reward of the final answer produced under current topology.
